SURIMI: Supervised Radio Map Augmentation with Deep Learning and a Generative Adversarial Network for Fingerprint-based Indoor Positioning

Indoor Positioning based on Machine Learning has drawn increasing attention both in the academy and the industry as meaningful information from the reference data can be extracted. Many researchers are using supervised, semi-supervised, and unsupervised Machine Learning models to reduce the positioning error and offer reliable solutions to the end-users. In this article, we propose a new architecture by combining Convolutional Neural Network (CNN), Long short-term memory (LSTM) and Generative Adversarial Network (GAN) in order to increase the training data and thus improve the position accuracy. The proposed combination of supervised and unsupervised models was tested in 17 public datasets, providing an extensive analysis of its performance. As a result, the positioning error has been reduced in more than 70% of them.

==> tables/tbl_cgan_parameters.tex <==
\begin{table}[!hbtp]
    \tabcolsep 4pt
    \caption{CNN-LSTM Parameter}
    \label{table:parameters}
    \centering
    \begin{threeparttable}
    \begin{tabular}{
    l
    l
    l
    l
    l
    l
    }
         \toprule
            &Layer
            &Parameter
            &Position
            &Floor
            &Building\\
         \midrule
\parbox[t]{2mm}{\multirow{12}{*}{\rotatebox[origin=c]{90}{TimeDistributed}}} &\multirow{3}{*}{Conv1D}&Filter&8&16&16\\
&&Activation&elu&relu&relu\\
&&kernel\_size&1&1&1\\
\cmidrule{2-6}
&MaxPooling1D&pool\_size&1&2&2\\
\cmidrule{2-6}
&Dropout&rate&0.5&0.5&0.5\\
\cmidrule{2-6}
&\multirow{4}{*}{Conv1D}&Filter&8&32&\\
&&Activation&elu&relu&\\
&&kernel\_size&1&1&\\
&&padding&same&same&\\
\cmidrule{2-6}
&MaxPooling1D&pool\_size&1&1&\\
\cmidrule{2-6}
&Dropout&rate&0.5&0.5&\\
\cmidrule{2-6}
&Flatten&&&&\\
\midrule
\multirow{3}{*}{\ac{lstm}}&&Units&40&50&40\\
&&Activation&elu&relu&relu\\
\midrule
\multirow{2}{*}{Dense}&&Units&3&CF&CB\\
&&Activation&elu&softmax&softmax\\

\bottomrule
%\multicolumn{6}{c}{Training parameters}\\
         \toprule
&&lr&0.0005&0.0001&0.0001\\
\multicolumn{2}{c}{Training parameters}&epochs&100&100&100\\
&&batch\_size&256&100&100\\
&&Optimizer&Adam&Adam&Adam\\
         \bottomrule
         
    \end{tabular}
    \begin{tablenotes}
        \item CF: Number of classes - Floors, CB: Number of classes - Buildings
        \end{tablenotes}
    \end{threeparttable}
\end{table}

==> tables/tbl_comparison_bck.tex <==
\begin{table*}[!hbtp]
    \tabcolsep 2pt
    
    \caption{Comparison Between \ac{knn} and the proposal indoor positioning framework (SURIMI) }
    \label{table:comparisonknn}
    \centering

    \begin{tabular}{l
    rr
    rrrccc
    cccc
    ccccc
    ccccc
    }
         \toprule
            &\multicolumn{2}{c}{Dim.}
            &\multicolumn{6}{c}{Baseline 1-NN}
            &\multicolumn{4}{c}{\ac{cnn}-\ac{lstm}}
            &\multicolumn{5}{c}{SURIMI M2}
            &\multicolumn{5}{c}{SURIMI M3}
            \\
         \cmidrule(rl){2-3}
         \cmidrule(rl){4-9}
         \cmidrule(rl){10-13} 
         \cmidrule(rl){14-18}
         \cmidrule(rl){19-23}
            Database
            &$\abs{\tau}$
            &$\abs{A}$
            &$\epsilon_{2D}$
            &$\epsilon_{3D}$
            &$\gamma$
            &$\iota$
            &$\tilde\epsilon_{2D}$
            &$\tilde\epsilon_{3D}$

            
            &$\tilde\epsilon_{2D}$
            &$\tilde\epsilon_{3D}$
            &$\gamma$
            &$\iota$
            
            &$\phi$
            &$\tilde\epsilon_{2D}$
            &$\tilde\epsilon_{3D}$
            &$\gamma$
            &$\iota$

            &$\phi$
            &$\tilde\epsilon_{2D}$
            &$\tilde\epsilon_{3D}$
            &$\gamma$
            &$\iota$\\
         \midrule
         \multicolumn{23}{c}{\ac{wifi} datasets}\\ 
         \midrule
DSI~1&1369&157&4.97&4.97&100\%&100\%&1&1&0.88&0.88&100\%&100\%&25712&0.74&0.74&100\%&100\%&24358&0.79&0.79&100\%&100\%\\
DSI~2&576&157&4.96&4.96&100\%&100\%&1&1&1.29&1.29&100\%&100\%&24350&0.98&0.98&100\%&100\%&23897&1.02&1.02&100\%&100\%\\
LIB~1&576&174&3.00&3.01&99.84\%&100\%&1&1&0.96&1.02&99.36\%&100\%&3712&0.94&0.95&98.85\%&100\%&54&0.94&0.98&99.07\%&100\%\\
LIB~2&576&197&4.00&4.18&97.67\%&100\%&1&1&0.73&0.74&99.42\%&100\%&969&0.76&0.77&98.33\%&100\%&118&0.80&0.86&99.62\%&100\%\\
MAN~1&14300&28&2.84&2.84&100\%&100\%&1&1&0.87&0.87&100\%&100\%&23578&0.87&0.87&100\%&100\%&24247&0.89&0.89&100\%&100\%\\
MAN~2&1300&28&2.47&2.47&100\%&100\%&1&1&0.98&0.98&100\%&100\%&11478&0.84&0.84&100\%&100\%&6505&0.86&0.86&100\%&100\%\\
%SIM&10710&8&3.08&3.08&100\%&100\%&1&1&0.83&0.83&100\%&100\%&&\\
TUT~1 &1476&309&8.59&9.55&90\%&100\%&1&1&0.88&0.81&93.27\%&100\%&4541&0.86&0.78&89.18\%&100\%&3526&0.83&0.76&91.63\%&100\%\\
TUT~2&584&354&13.00&15.11&71.02\%&100\%&1&1&1.05&0.90&90.34\%&100\%&613&1.03&0.89&89.77\%&100\%&45&1.14&0.98&90.91\%&100\%\\
TUT~3&697&992&8.89&9.58&91.42\%&100\%&1&1&1.39&1.30&91.98\%&100\%&1248&1.28&1.20&90.66\%&100\%&369&1.32&1.23&92.05\%&100\%\\
TUT~4&3951&992&6.15&6.40&95.40\%&100\%&1&1&1.02&0.98&96.41\%&100\%&5502&1.03&1.00&96.84\%&100\%&184&1.16&1.13&96.70\%&100\%\\
TUT~5&446&489&6.39&6.92&88.39\%&88.39\%&1&1&1.74&1.62&97.56\%&100\%&596&1.74&1.62&98.57\%&100\%&1232&1.49&1.38&99.29\%&100\%\\
TUT~6&3116&652&2.07&2.08&99.95\%&100\%&1&1&2.62&2.62&99.90\%&100\%&6329&2.10&2.10&99.39\%&100\%&186&2.60&2.60&99.96\%&100\%\\
TUT~7&2787&801&2.23&2.62&99.12\%&100\%&1&1&2.32&1.98&98.06\%&100\%&809&2.18&1.86&98\%&100\%&82&2.17&1.86&98.32\%&100\%\\
\midrule
\multicolumn{23}{c}{BLE datasets} \\
\midrule
UJIB~1&1632&24&3.07&3.07&100\%&100\%&1&1&0.93&0.93&100\%&100\%&1990&0.95&0.95&100\%&100\%&1990&0.95&0.95&100\%&100\%\\
UJIB~2&816&22&4.25&4.25&100\%&100\%&1&1&0.93&0.93&100\%&100\%&1990&0.93&0.93&100\%&100\%&1990&0.90&0.90&100\%&100\%\\
\midrule
Avg.&&&&&95.37\%&99.22\%&1&1&1.24&1.19&96.90\%&100\%&&1.15&1.10&&100\%&&1.19&1.15&&100\%\\
         \bottomrule
    \end{tabular}
\end{table*}

==> tables/tbl_full_comparison.tex <==
\begin{table*}[!hbtp]
    \tabcolsep 3.5pt
    
    \caption{Comparison among the 1-NN baseline, CNN-LSTM  and the proposed  models. $\phi$ stands for the number of new fingerprints.}
    \label{table:comparisonknn}
    \centering
    %\begin{threeparttable}
    \begin{tabular}{
    l
    rrr
    rrcc
    ccc
    cccc
    cccc
    }
         \toprule
            &\multicolumn{3}{c}{Dim.}
            &\multicolumn{5}{c}{Baseline 1-NN}
            &\multicolumn{3}{c}{\ac{cnn}-\ac{lstm}}
            &\multicolumn{4}{c}{SURIMI M2}
            &\multicolumn{4}{c}{SURIMI M3}
            \\
         \cmidrule(rl){2-4}
         \cmidrule(rl){5-9}
         \cmidrule(rl){10-12} 
         \cmidrule(rl){13-16}
         \cmidrule(rl){17-20}
            Database
            &$\abs{\tau}$
            &$\abs{A}$
            &$\delta_{fp}$
            
            &$\epsilon_{2D}$
            &$\epsilon_{3D}$
            &$\gamma$
            &$\tilde\epsilon_{2D}$
            &$\tilde\epsilon_{3D}$

            
            &$\tilde\epsilon_{2D}$
            &$\tilde\epsilon_{3D}$
            &$\gamma$
            
            &$\phi$
            &$\tilde\epsilon_{2D}$
            &$\tilde\epsilon_{3D}$
            &$\gamma$

            &$\phi$
            &$\tilde\epsilon_{2D}$
            &$\tilde\epsilon_{3D}$
            &$\gamma$\\
         \midrule
         \multicolumn{20}{c}{\ac{wifi} datasets}\\ 
         \midrule
DSI~1&1369&157&6&4.97&4.97&100\%&1&1&0.88&0.88&100\%&25712&0.74&0.74&100\%&24358&0.79&0.79&100\%\\
DSI~2&576&157&2-3&4.96&4.96&100\%&1&1&1.29&1.29&100\%&24350&0.98&0.98&100\%&23897&1.02&1.02&100\%\\
LIB~1&576&174&12&3.00&3.01&99.84\%&1&1&0.96&1.02&99.36\%&3712&0.94&0.95&98.85\%&54&0.94&0.98&99.07\%\\
LIB~2&576&197&12&4.00&4.18&97.67\%&1&1&0.73&0.74&99.42\%&969&0.76&0.77&98.33\%&118&0.80&0.86&99.62\%\\
MAN~1&14300&28&110&2.84&2.84&100\%&1&1&0.87&0.87&100\%&23578&0.87&0.87&100\%&24247&0.89&0.89&100\%\\
MAN~2&1300&28&10&2.47&2.47&100\%&1&1&0.98&0.98&100\%&11478&0.84&0.84&100\%&6505&0.86&0.86&100\%\\
%SIM&10710&8&3.08&3.08&100\%&100\%&1&1&0.83&0.83&100\%&100\%&&\\
TUT~1 &1476&309&1&8.59&9.55&90\%&1&1&0.88&0.81&93.27\%&4541&0.86&0.78&89.18\%&3526&0.83&0.76&91.63\%\\
TUT~2&584&354&1&13.00&15.11&71.02\%&1&1&1.05&0.90&90.34\%&613&1.03&0.89&89.77\%&45&1.14&0.98&90.91\%\\
TUT~3&697&992&1&8.89&9.58&91.42\%&1&1&1.39&1.30&91.98\%&1248&1.28&1.20&90.66\%&369&1.32&1.23&92.05\%\\
%TUT~4&3951&992&1&6.15&6.40&95.40\%&1&1&1.02&0.98&96.41\%&5502&1.03&1.00&96.84\%&184&1.16&1.13&96.70\%\\
TUT~5&446&489&1&6.39&6.92&88.39\%&1&1&1.74&1.62&97.56\%&596&1.74&1.62&98.57\%&1232&1.49&1.38&99.29\%\\
TUT~6&3116&652&1&2.07&2.08&99.95\%&1&1&2.62&2.62&99.90\%&6329&2.10&2.10&99.39\%&186&2.60&2.60&99.96\%\\
TUT~7&2787&801&1&2.23&2.62&99.12\%&1&1&2.32&1.98&98.06\%&809&2.18&1.86&98\%&82&2.17&1.86&98.32\%\\
\midrule
\multicolumn{20}{c}{BLE datasets} \\
\midrule
UJIB~1&1632&24&30 \& 36&3.07&3.07&100\%&1&1&0.93&0.93&100\%&1990&0.95&0.95&100\%&1990&0.95&0.95&100\%\\
UJIB~2&816&22&24&4.25&4.25&100\%&1&1&0.93&0.93&100\%&1990&0.93&0.93&100\%&1990&0.90&0.90&100\%\\
\midrule
Avg.&&&&&&95.53\%&1&1&1.25&1.20&97.84\%&&1.16&1.10&97.34&&1.20&1.15&97.90\%\\
         \bottomrule
    \end{tabular}
    %\end{threeparttable}
    %\begin{tablenotes}
    %\item $\phi$: number of new fingerprints. 
    %\end{tablenotes}
\end{table*}

==> tables/tbl_results_full.tex <==
\begin{table*}[!hbtp]
    \tabcolsep 2.35pt
    
    \caption{Main results}
    \label{table:comparison}
    \centering
    \begin{threeparttable}
    \begin{tabular}{l
    rrrr
    rrcc
    |rrcc
    crrcc
    crrcc
    crrcc
    }
         \toprule
            &\multicolumn{4}{c}{CNNLoc \cite{song2019cnnloc}}
            &\multicolumn{4}{c}{CCPos \cite{quin2021ccpos}}
            &\multicolumn{4}{c}{\ac{cnn}-\ac{lstm}}
            &\multicolumn{5}{c}{CL-c\ac{gan} BL}
            &\multicolumn{5}{c}{CL-c\ac{gan} FL}
            &\multicolumn{5}{c}{CL-c\ac{gan} FD}
            \\
         \cmidrule(rl){2-5} 
         \cmidrule(rl){6-9} 
         \cmidrule(rl){10-13}
         \cmidrule(rl){14-18}
         \cmidrule(rl){19-23}
         \cmidrule(rl){24-28}
            Database 
            &$\epsilon_{2D}$
            &$\epsilon_{3D}$
            &$\gamma$
            &$\iota$
            
            &$\epsilon_{2D}$
            &$\epsilon_{3D}$
            &$\gamma$
            &$\iota$

            &$\epsilon_{2D}$
            &$\epsilon_{3D}$
            &$\gamma$
            &$\iota$
            
            &$\eta$
            &$\epsilon_{2D}$
            &$\epsilon_{3D}$
            &$\gamma$
            &$\iota$
            
            &$\eta$
            &$\epsilon_{2D}$
            &$\epsilon_{3D}$
            &$\gamma$
            &$\iota$
            
            &$\eta$
            &$\epsilon_{2D}$
            &$\epsilon_{3D}$
            &$\gamma$
            &$\iota$\\
         \midrule
         \multicolumn{28}{c}{\ac{wifi} data sets}\\ 
         \midrule
\textasteriskcentered \textbullet UJIIndoorLoc  \cite{}&11.78&13.08&96.03\%&100\%&12.4& &95.3\%&99.6\%& 10.91 & 10.95 &95.32\%&100\%&-&-&-\\
\textbullet Tampere \cite{} &10.88&&94.22\%&-& & &-& &11.33&11.44&91.97\%&-&10.00&10.09&92.30\%&-&\\
\textbullet UTSIndoorLoc \cite{song2019cnnloc}&7.60&&94.57\%&-& & &-& &8.30&8.72&90\%&-&-\\
%Alcalá 2017 Tutorial \cite{montoliu2017indoorloc}& 4.62 & &-&-& 1.05 & & & & &-&-&-&-\\

\bottomrule
    \end{tabular}

       \textasteriskcentered Multi-building dataset, 
       \textbullet Multi-floor dataset, 
       BL: c\ac{gan} trained by building, 
       FL: c\ac{gan} trained by floor, 
       FD: c\ac{gan} full dataset.
       
    \end{threeparttable}
\end{table*}

==> tables/tbl_test.tex <==
\begin{table}[!hbtp]
    \tabcolsep 2pt
    \caption{Training c\ac{gan} by}
    \label{table:test}
    \centering
    \begin{threeparttable}
    \begin{tabular}{l
    S
    S
    S
    S
    S
    S
    }
         \toprule
            Database 
            &$\delta$
            &$\gamma$
            &$\epsilon_{2D}$
            &$\epsilon_{3D}$
            &$\gamma$
            &$\iota$\\
         \midrule
         \multicolumn{7}{c}{\ac{wifi} data sets}\\
         \midrule
UJIIndoorLoc & 1369 & 157 & 2\\
Tampere & 576 & 157 & 3 \\
UTSIndoorLoc & 576 & 174 & 1 \\
Alcalá 2017 Tutorial & 576 & 197 & 1 \\
\midrule
\multicolumn{7}{c}{\ac{ble} data sets}\\
\midrule
UEXB~1 &417&30& 2 \\
UEXB~2 &552&30 & 2 \\
UEXB~3 &240&30 & 1 \\
         \bottomrule
    \end{tabular}
    \end{threeparttable}
    %\tablefootnote{* DSI - U. , LIB - U. Jaume I, MAN - U. Mannheim, TUT - Tampere U. } 
\end{table}

==> zz_ORCID.tex <==
\usepackage{scalerel}
\usepackage{tikz}
\usetikzlibrary{svg.path}

\definecolor{orcidlogocol}{HTML}{A6CE39}
\tikzset{
    orcidlogo/.pic={
        \fill[orcidlogocol] svg{M256,128c0,70.7-57.3,128-128,128C57.3,256,0,198.7,0,128C0,57.3,57.3,0,128,0C198.7,0,256,57.3,256,128z};
        \fill[white] svg{M86.3,186.2H70.9V79.1h15.4v48.4V186.2z}
        svg{M108.9,79.1h41.6c39.6,0,57,28.3,57,53.6c0,27.5-21.5,53.6-56.8,53.6h-41.8V79.1z M124.3,172.4h24.5c34.9,0,42.9-26.5,42.9-39.7c0-21.5-13.7-39.7-43.7-39.7h-23.7V172.4z}
        svg{M88.7,56.8c0,5.5-4.5,10.1-10.1,10.1c-5.6,0-10.1-4.6-10.1-10.1c0-5.6,4.5-10.1,10.1-10.1C84.2,46.7,88.7,51.3,88.7,56.8z};
    }
}

\newcommand\orcidicon[1]{\href{https://orcid.org/#1}{\mbox{\scalerel*{
                \begin{tikzpicture}[yscale=-1,transform shape]
                \pic{orcidlogo};
                \end{tikzpicture}
            }{|}}}}

\usepackage[bookmarks=false,hidelinks]{hyperref} %<--- Load after everything else

